Distributional Individual Fairness in Clustering

In this paper, we initiate the study of fair clustering that ensures distributional similarity among similar individuals. In response to improving fairness in machine learning, recent papers have investigated fairness in clustering algorithms and have focused on the paradigm of statistical parity/group fairness. These efforts attempt to minimize bias against some protected groups in the population. However, to the best of our knowledge, the alternative viewpoint of individual fairness, introduced by Dwork et al. (ITCS 2012) in the context of classification, has not been considered for clustering so far. Similar to Dwork et al., we adopt the individual fairness notion which mandates that similar individuals should be treated similarly for clustering problems. We use the notion of $f$-divergence as a measure of statistical similarity that significantly generalizes the ones used by Dwork et al. We introduce a framework for assigning individuals, embedded in a metric space, to probability distributions over a bounded number of cluster centers. The objective is to ensure (a) low cost of clustering in expectation and (b) individuals that are close to each other in a given fairness space are mapped to statistically similar distributions. We provide an algorithm for clustering with $p$-norm objective ($k$-center, $k$-means are special cases) and individual fairness constraints with provable approximation guarantee. We extend this framework to include both group fairness and individual fairness inside the protected groups. Finally, we observe conditions under which individual fairness implies group fairness. We present extensive experimental evidence that justifies the effectiveness of our approach.

==> source/intro_nips.tex <==
\section{Introduction}


% 1. Fairness in ML in general
Machine learning based systems are increasingly being deployed in tasks that involve making decisions about individuals. In recent years, it has been demonstrated that such systems might suffer from inherent biases in favor or against a certain group of the population under consideration. 
Prominent examples include face recognition tools~\cite{Harwell2019}, targeted ad placement~\cite{speicher2018potential}, issuing home loans~\cite{bartlett2019consumer},
predicting recidivism~\cite{propublica,chouldechova2017fair} and gender inequality at workplace~\cite{datta2015automated,Miller2015}. Clustering technique is not an exception. With wide application of clustering algorithms in domains such as recommender systems \cite{sarwar2002recommender}, customer segmentation \cite{chen2012data}, feature generation \cite{larsen1999fast,kg2006feature}, %\yl{the 2006 paper particularly mentioned fuzzy k means for feature extraction}
targeted advertisement \cite{aggarwal2004method} etc., it is important to guarantee that the outcome of clustering algorithms designed are fair to individuals. 


% 2. Notion of Fairness
To address these issues, two broad categories of fairness notions have emerged: {\em group} fairness (or {\em statistical} fairness)
and {\em individual} fairness. In the former, the {\em odds} are required to be approximately equalized 
across various protected groups in the 
population. This solution concept has been successfully implemented to improve the fairness guarantee of a clustering algorithm \cite{CKLV18,RS18,Bercea2018,bera19,Ahmadian:2019}. 


However, forcing {\em group} fairness can lead to {\em disparate treatment} 
of similar individuals or can even open up the possibility of gerrymandering by unfairly targeting a subgroup of a protected group --- see~\cite{kearns2018preventing},~\cite{kearns2019empirical}. Figures~\ref{fig:unfairBoundary} and \ref{fig:combined_fairness} %\yl{double check the ways we call figures. } illustrate these effects. 
Taking Figure~\ref{fig:combined_fairness}, for example,
group fairness demands that, in each cluster at least one third of the points must be circles (red). Naturally, two of the points from 
the set $R_{L}$, marked with oval, needs to be assigned to the cluster on the right, $C_R$. However, this would violate {\em individual}
fairness between these points and the remaining points in $R_{L}$. %\yl{Add discussions back about the figures.} 
Therefore it is important to look beyond the
notion of {\em group} fairness. 


\begin{figure}[!ht]
\centering
\begin{minipage}[b]{.35\textwidth}
\centerline{\includegraphics[height=0.8\linewidth,width=1\linewidth]{images/illu.eps}}
\caption{A simple problem to illustrate the possibility of harming the individuals (on the boundaries of three clusters) via off-the-shelf clustering method.}
\label{fig:unfairBoundary}
\end{minipage}\qquad
\begin{minipage}[b]{.5\textwidth}
\centering
\includegraphics[width=1\linewidth,trim={1in 4in 3in 1in},clip]{images/gf_if.pdf}
\caption{Group fairness might affect Individual Fairness. Moving circled red points from $R_L$ to Right cluster would violate {\em individual}
fairness constraints between these points and the remaining points in $R_{L}$ }
\label{fig:combined_fairness}
\end{minipage}
\end{figure}


%Thus, for any machine learning model, 
In a seminal work, Dwork~\etal~\cite{dwork2012fairness} propose the notion of {\em individual fairness} 
in classification. Assuming prior knowledge of a {\em similarity measure} between the 
individuals in the training set $V$, defined by a metric $d: V\times V\rightarrow {\mathbb R}$, 
an {\em individually } fair classifier (1) maps each point $x$ in the training set $V$
to a distribution $\mu_x$ over the set of possible outcomes, and (2) ensures that for every pair $x$ and $y$, 
the statistical distance $D$ between $\mu_x$ and $\mu_y$ is at most $d(x,y)$ for some suitably chosen distance measure $D$. 
In particular, they consider two statistical distance metrics --- the {\em total variation distance norm} and {\em the relative
$\ell_{\infty}$ metric}. To the best of our knowledge, the above notion of individual fairness has not been explored so far in {\em clustering}. Our goal is to provide such a treatment to complement the literature. %More formally:
%In the latter, every pair of {\em similar} individuals are mandated to be treated {\em similarly}.
%Ensuring {\em group} fairness is computationally easier and has been widely studied.\syam{This might piss group fairness folks}



% 3. Individual fairness in clustering
 
%Although the notion of {\em group} fairness has been studied extensively in the context of clustering~\cite{CKLV18,Backurs2019,bera19,huang2019coresets,Kleindessner2019}, 


%\emph{In this paper, we formalize the notion of individual fairness in clustering and 
%give an algorithmic framework with provable guarantees for achieving the same. We also 
%study the notion of combined fairness that includes both group fairness and individual fairness,
%and extend our framework to handle the same.}

% 4. Individual fairness in general
% (see~\Cref{sec:prelim}), were considered.

% 4. Individual fairness in clustering


\noindent
{\bf Our notion : Individual fairness in $k$-clustering.}
In $k$-clustering problems, for example $k$-means, $k$-median, $k$-center and so on, the input consists of a set of
points $V$ embedded in a known metric space . The goal
is to partition the points into $k$ clusters while minimizing some distanced-based objective function. 
It is natural to expect that individuals which are `close' to each other in this space would be assigned to the same cluster by any reasonable clustering heuristic. However, as demonstrated in Fig.~\ref{fig:unfairBoundary}, any deterministic clustering method can potentially affect similar individuals that lie at the boundary of the clusters. In order to overcome this issue, we propose the natural idea of randomized assignment as part of our solution concept. Inspired by ideas from Dwork et al.~\cite{dwork2012fairness}, our framework produces a mapping of each point in $V$ to a distribution over $k$ centers, $\calC$, while minimizing the expected clustering cost.

In this work, we ensure individual fairness between points through distributional similarity. In other words, we require the statistical distance between the output distributions of two points in $V$ to closely mirror their actual distance in the metric space. In particular, we use $f$-divergence, introduced in~\cite{csiszar1964informationstheoretische,morimoto1963markov,ali1966general}, as the similarity measure between two distributions. This is analogous to the definition of individual fairness in classification by Dwork et al.~\cite{dwork2012fairness}. However, in classification, either one has to assume the knowledge of a similarity metric as side information or she faces the non-trivial task of computing~\cite{} or learning the same~\cite{dworkICML}. On the other hand, distance metric is an essential parameter in clustering problems and thus distance-based definition of individual fairness seems natural in this context. Our framework, however, is flexible enough to handle the situation where one might want to use two different distance metrics for the objective function and fairness constraints. We provide constant factor approximation algorithms for a general class of $k$-clustering problems with $\ell_p$-norm objectives ($k$-means, $k$-median, $k$-center are special cases) that ensure individual fairness.  
 As explained above, our solution is probabilistic. It might be noted that a single realization according to the distributions that our algorithm produces might still be unfair to a pair of individuals which are close to each other in the similarity metric space. However, upon repeated trials, they would be assigned to the same cluster with high probability. Our experiments on real datasets conform to this as demonstrated in Appendix~\ref{}.

 \syam{Shall we shorten this part ?} Closest to our idea is the soft $k$-means clustering~\cite{skm-lecture-notes} \syam{cite the books} which outputs a distribution over the centers $\calC$ for each point in $V$. In particular, for some fixed stiffness parameter $\beta$, the probability $\mu_{x}(i)$ of assigning $x\in V$  to $c_i\in \calC$ is given by $\frac{ e^{-\beta d(c_i,x)^ 2} } { \sum_{\ell = 1}^{k} e^{-\beta d(c_{\ell},x)^ 2} }$. Besides lacking in theoretical guarantees, such an approach fails to achieve the correct trade-off between fairness and cost as we show  experimentally in~\Cref{sec:exp}. 

 
 
 \noindent
{\bf Combining {\em group} fairness with {\em individual}  fairness.}
Roughly speaking,
group fairness requires that each protected group
in the population is  'well-represented' in each cluster.  %Although group fairness appears to be a desirable property of learning algorithms, the inadequacy of this notion as an exclusive definition of fairness has been demonstrated in several instances~\cite{}, particularly from the point of view of individuals in a population. We exemplify this further through the toy example given in Figure~\ref{fig:combined_fairness}. 
Thus we ask - {\em can we combine the two notions of fairness in the context of clustering problems?}. %Recall that we are assigning each point $x$ to a distribution $\mu_x$ over the cluster centers. Hence, we slightly modify the definition of group fairness by considering the expected representation of protected groups in each cluster. 
A first attempt would be to simply impose group fairness constraints along with the individual fairness constraints on {\em every pair of points}. Such a stringent requirement can potentially lead to trivial and expensive solutions as elaborated in Appendix~\ref{}. We alleviate this issue by enforcing individual fairness among points only inside the same protected group. We give constant factor approximation algorithms for $k$-clustering problems that ensure both statistical and individual fairness.
%\syam{Need to address the case of overlapping groups since a trivial case where all points belong to a single group in addition to being part of other groups will kill this approach. Reviewer3 had pointed this out} 

%Such a setting lends itself naturally to a definition of {\em individual}
%fairness constraints on the basis of distance between points in the metric space, as elaborated next.



%Through the development of our solution concept, we notice that a certain form of randomness will be needed in the algorithm's output to guarantee individual fairness. This was also pointed out in~\cite{dwork2012fairness}. We first modify the definition of $k$-clustering problems slightly to incorporate randomness in the output. 

%The goal is to form a set of $k$ clusters around centers $\calC=\{c_1, c_2,\ldots, c_k\}$. 
%We define a mapping $\mu : V \rightarrow \Delta(\calC)$, where $\Delta$ is the set of probability distributions over the open centers. We use $d(x, c)$ to denote the distance between point $x \in V$ and center $c \in \calC$. Let $r_{\mu, \calC}(x)$ denote the distance between point $x$ and farthest center $c^* \in \calC$ such that $\mu_x(c^*) \ne 0$. 
%Then, the $k$-center, $k$-median and $k$-means objective functions are $\max_{x\in V} r_{\mu,\calC}(x)$, 
%$\sum_{x\in V} \mathbb{E}_{c\sim\mu_x}[d(x, c)]$, and $\left(\sum_{x\in V} \mathbb{E}_{c\sim\mu_x}[d(x, c)^2]\right)^{1/2}$ respectively. 
%In order to enforce individual fairness, we use $f$-divergence,
%formally introduced in~\cite{csiszar1964informationstheoretische,morimoto1963markov,ali1966general}, as a similarity measure between two distributions. Our fairness requirement mandates that $f$-divergence between two distributions of the output solution, $\mu_x$ and $\mu_y$ must be upper bounded by the distance $d(x,y)$ up to normalization, for all points $x,y\in V$. (see~\Cref{sec:prelim} for a formal statement)

%5. Our problem formulation
% In recent years a significant body of work has addressed these issues~\cite{TODO}. 
% Algorithms have been proposed that aim to ensure fairness in various aspects of machine learning, like supervised learning \cite{}, unpsupervised learning \cite{}, sequential learning \cite{} and more. Much of these papers have focused on providing {\em group level fairness} guarantee. This entails, for example, working under the Disparate Impact (DI) Doctrine which asserts that individuals belonging to various protected groups within a population should be treated uniformly by any algorithmic decision. However, in the seminal paper~\cite{dwork2012fairness}, the authors raise the concern that algorithms that ensure group fairness may potentially treat a pair of similar individuals quite differently. We mention two such possible scenarios. 
% \begin{itemize}
%     \item Guaranteeing group level fairness may bring disparity between two individuals in the same protected group~\cite{}. 
%     \item It opens up possibilities of gerrymandering by creation of unfair groups. A machine learning model might look fair for the protected groups, but turns out to be unfair for a subgroup of a specific group.
% \end{itemize}
% Impact of fairness on classfier


% However, as we show experimentally in Section~\ref{sec:exp}, 
% \begin{figure}[h]
% \centerline{\includegraphics[width=1\columnwidth]{images/illu.eps}}
% \caption{A simple problem to illustrate the possibility of harming the individuals (on the boundaries of three clusters) via off the shelf clustering method.
% }
% \label{table:NoiseReducesAccuracy}
% \end{figure}

% \noindent
% {\bf Individual fairness in classification.} In~\cite{dwork2012fairness}, the authors propose a notion of {\em individual fairness} in the context of classification which is an important problem in the paradigm of supervised learning. The model assumes a {\em similarity measure} between the individuals in the training set $V$, defined by a metric $d: V\times V\rightarrow {\mathbb R}$.  

% \begin{enumerate}
%     \item {\bf Randomized Classification.} For each point $x\in V$, the algorithm should output a distribution $\mu_x$ on the set of possible outcomes.
    
%     \item {\bf $(D,d)$-Lipschitz.} For a suitably chosen measure of statistical distance $D$ between any two distributions $\mu_x$ and $\mu_y$, $D(\mu_x, \mu_y) \leq d(x,y), \forall x,y\in V $
%     \end{enumerate}

% The authors propose two such measures as follows.

% \begin{enumerate}
%     \item {\bf Total variation norm}. Given any two distributions $\mu_x$ and $\mu_y$ on the set of outcomes $A$, total variation norm is defined by
%     $$ D_{tv}(\mu_x, \mu_y) = \frac{1}{2}\sum_{a\in A}|\mu_x(a) - \mu_y(a)| $$
    
%     \item {\bf Relative $\ell_{\infty}$ metric.} 
%      $$D_{\infty}(\mu_x, \mu_y) = \text{sup}_{a\in A}\log \Bigg[\max\left\{\frac{\mu_x(a)}{\mu_y(a)}, \frac{\mu_y(a)}{\mu_x(a)}\right\}\Bigg]$$
% \end{enumerate}

% A series of papers build upon this idea and attempt to extend and improve upon its various aspects, as elaborated in Section~\ref{sec:related}.
%\subsection{Our contributions}
%{\bf Our contribution - Individual fairness in clustering.} 
%Somewhat surprisingly, the study of individual fairness has been restricted to supervised learning thus far, to the  best of our knowledge. 
% On the other hand, unsupervised learning observes fundamental roles in applications such as feature generation, targeted advertisement etc. Therefore it is important to guarantee that the outcome of algorithms designed under such paradigms will produce fair representation for individuals. 
%In this paper, we provide the \emph{ first set of results for individually fair clustering} - one of the fundamental problems in unsupervised learning. 
% We observe that in a typical clustering setting, the input consists of points embedded in a known metric space. 
% As elaborated on subsequently, such a setting lends itself  naturally to a definition of individual fairness constraints on the basis of distance between points. 
% We use generic measures to capture the difference between the clustering outcomes assigned to each pair of points.
Our main contributions can be summarized as follows:

\squishlist
    \item {\bf Distributional Individual Fairness for Clustering :} We introduce distributional individual fairness for $\ell_p$-norm clustering problems using a general family of divergence functions.
    \item  {\bf Approximation algorithms for Individually Fair Clustering} : We provide a generic solution template that adapts any algorithm for $\ell_p$-norm clustering objective to an individually fair solution. In particular, we give an algorithm for the individually fair $\ell_p$-norm $k$-clustering problem that achieves a constant factor approximation guarantee (Theorem~\ref{thm:individual_fairness}).  
    \item {\bf Algorithms for Combined Fairness} : We show connections between individual fairness and group fairness, and extend our solution to combine the two paradigms. We show that our framework can be seamlessly combined with ideas developed in~\cite{bera19} to give a constant factor approximation algorithm that guarantees both group fairness (in expectation) and individual fairness among members of the same group (Theorem~\ref{thm:combined_fairness}). Further, similar in spirit to Dwork et al~\cite{dwork2012fairness}, we show that when the protected groups have statistically similar representation in the population, individual fairness implies group fairness (Theorem~\ref{}). 
   % \item We complement our positive results by proving that clustering under individual fairness constraints is NP-hard for the special case of $k$-center.(\syam{With the correct definition of $k$-center, this becomes trivial now. I guess we can just mention this.})
\squishend
    We provide extensive empirical evidences to support the effectiveness of our method.\footnote{We are contributing our code to the community.} Experiments show that our method achieves objective cost much better than predicted by our theoretical analysis, while respecting individual fairness.   
    
    %\syam{Shall we add one or two sentences about the experiments here already }
%\end{enumerate}


% {\bf Overview of Approach.} We modify the definition of $k$-clustering problems slightly to incorporate randomness in the output. The goal is to form a set of $k$ clusters around centers $\calC=\{c_i, i=1,2,\cdots k\}$. Further, we shall define a mapping $\mu : V \rightarrow \Delta(\calC)$, where $\Delta$ is a set of probability distributions on the set of open centers. The expected distance for any point $x\in V$ is now naturally defined as 

% $$\mathbb{E}_{c\sim\mu_x} d(x, c)\,. $$
% We use $d_{\mu,\calC}(x)$ to denote the expected distance 
% of the point $x$ from the set of centers $\calC$ following the
% distribution $\mu_x$.

% Then the $k$-center, $k$-median and $k$-means objective functions are respectively $\max_{x\in V} d_{\mu,\calC}(x)$, 
% $\sum_{x\in V} d_{\mu,\calC}(x)$, and $\sum_{x\in V} d_{\mu,\calC}(x)^2$. In order to enforce individual fairness, we use $f$-divergence, formally introduced in~\cite{RubnerTG98}, as a similarity measure between two distributions. Our fairness requirement mandates that $f$-divergence between two distributions of the output solution, $\mu_x$ and $\mu_y$ must be upper bounded by the distance $d(x,y)$ up to normalization, for all points $x,y\in V$.
 




% In the classical setting, 
%each individual belongs to a fixed cluster; in our setting, the cluster membership of $x$ is
%implicitly defined by the distribution $\mu_x$. Hence, to define {\em group} fairness, we 
%consider the expected representation of protected groups in each cluster.

%Can we simultaneously achieve {\em group} fairness and {\em individual} fairness? Observe that,
%by choosing $\mu$ to be the uniform distribution for each point, we can trivially satisfy both the
%fairness concepts. However, as we demonstrate in~\Cref{fig:combined_fairness}, imposing {\em individual}
%fairness constraints for each pair of points is going to lead to trivial and very expensive solutions.
%Dwork~\etal~\cite{dwork2012fairness} make similar observations in the context of 
%classification problems. Inspired by ~\cite{dwork2012fairness}, when combining {\em group} fairness
%with {\em individual} fairness, we only demand a pair of points within the same protected group to
%be treated similarly (see~\Cref{sec:prelim} for formal definition).


% \begin{figure}[!ht]
% \begin{center}
% \centerline{\includegraphics[width=1\columnwidth,trim={1in 4in 3in 1in},clip]{images/gf_if.pdf}}
% \caption{Can we achieve both individual fairness and group fairness? In this toy example, assume
% group fairness demands that, in each cluster at least one third of the points must be circles (red). Naturally, two of the points from 
% the set $R_{L}$, marked with oval, needs to be assigned to the cluster on the right, $C_R$. However, this would violate {\em individual}
% fairness constraints between these points and the remaining points in $R_{L}$. }
% \label{fig:combined_fairness}
% \end{center}
% \end{figure}





==> source/relation.tex <==
\section{The special Individual Fairness to Group Fairness}
\label{sec:ind}

We explore the connection between the notion of 
individual fairness and group fairness. In particular, we are interested in 
finding conditions under which individually fair clustering solutions guarantees group fairness.
%characterization of the protected groups (in terms of the 
%underlying metric space)
%that will ensure any individually fair clustering solution
%guarantees group fairness as well. 
%Such connections are well-known in the context
%of classification problems~\cite{dwork2012fairness}. We show that similar connections
%exist in the clustering context. 
%We define a quantity {\em maximum additive violation}, and denote it as $\MAD$,
%which captures the unfairness of the clusters for each protected group. This quantity helps us establish a connection between group fairness and individual fairness. Recall that,
%a solution to the \kfp instance assigns to each point $x\in V$ a distribution $\mu_x$ over the set of
%cluster centers $\calC$. For
%each protected groups $G_1,G_2,\ldots,G_{\ell}$, let $p_r= |G_r|/|V|$ for each $r\in [\ell]$.
%Then, for the protected group $G_r$, we define $\MAD_r$ as follows:
%\begin{align}
%    \MAD_r = \max_{i \in \calC} \left|  \sum_{j\in G_r} \mu_{x}(i) - p_r\sum_{j\in V} \mu_{x}(i)\right|
%\end{align}
%To elucidate further on this definition, note that in the entire population,
%$p_r$ fraction of the points belong to group $G_r$, and hence, we expect that
%each cluster will have the same proportional representation for group $G_r$. 
%The notion of $\MAD_r$ captures the additive deviation from this expected number.
%We remark here that our notion of $\MAD_r$ is consistent with the 
%most general group fairness constraints defined in prior works~\cite{bera19,Bercea2018}. 
%Indeed, the $(\alpha,\beta)$-group fairness formulation~\cite{bera19} aims at 
%providing a desired bound on the quantity $\MAD_r$.
For each protected group $G_r$, we define a distribution
$\nu_{G_r}$ as a uniform distribution over the set of points in $G_r$.
In particular, $\nu_{G_r}(x) = 1/|G_r|$ if $x\in G_r$, and $0$ otherwise.
Let $\nu_V$ be the uniform distribution over the set of all points:
$\nu_V(x) = 1/|V|$ for all $x\in V$. Let $d_{\EM}(S,T)$ be the 
Earthmover's distance between the distribution $S$ and $T$, introduced formally in~\cite{RubnerTG98}.
Our main result of this section is the following lemma, proof of which we defer to~\Cref{appendix:relation}.
\begin{restatable}{lemma}{relation}
\label{lem:relation}
Let $(\calC, {\mu})$ be any feasible solution to the \kfp problem 
instance with $D_f$ as the statistical similarity measure. Further suppose the $f$-divergence $D_f(\mu_x||\mu_y) \geq D_{\TV}(\mu_x, \mu_y)$ for all pair of points $x,y\in V$. 
Then, For each group $G_r$, $\MAD_r \leq |G_r| \cdot d_{\EM}(\nu_{G_r},\nu_V)$
\end{restatable}
% \begin{lemma}
% \label{lem:relation}
% Let $(\calC, {\mu})$ be any feasible solution to the \kfp problem 
% instance with $D_f$ as the statistical similarity measure. Further suppose the $f$-divergence $D_f(\mu_x||\mu_y) \geq D_{\TV}(\mu_x, \mu_y)$ for all pair of points $x,y\in V$. 
% Then, For each group $G_r$, $\MAD_r \leq |G_r| \cdot d_{\EM}(\nu_{G_r},\nu_V)$
% \end{lemma}
\begin{comment}
The first idea is to define bias for each protected group as the absolute 
difference between the expected fraction of points to the actual fraction 
of points over all the clusters. Formally, we define bias for the group $G_r$, denoted as $\eps_r$, as follows:
\begin{align}
\MAD_r = \max_{i\in [k]} \left|\frac{\sum_{j\in G_{r}} \mu_{x}(i)}{ \sum_{j\in V}\mu_{x}(i)} - p_r\right|
\end{align}

This definition of bias capture the notion of $(\alpha,\beta)$-statistical fairness formulation. For each group $G_{r}$,  set $\alpha_r = p_r + \eps_r$
and $\beta_r = p_r - \eps_r$. 

\textcolor{red}{Notes: In the definition of bias, we have used absolute value.
However, I believe we can remove it. The earthmover distance is asymmetric,
and by considering $d_{\EM}(\mu_{G_r},\mu_V)$ and $d_{\EM}(,\mu_V,\mu_{G_r})$
separately, we can probably capture both the positive and negative bias.}
\end{comment}
